Subspace-Aware Sparse Autoencoders for Effective Mechanistic Interpretability

Sparse Autoencoders (SAEs) are widely used for mechanistic interpretability in large language models, yet their standard formulation assigns each latent feature a single decoder direction, implicitly assuming features to be one-dimensional. We show that this assumption can induce feature splitting when model features are multi-dimensional. Geometrically, accurately reconstructing a feature under a fixed co-activation budget can require exponentially many decoder directions as its dimension grows. From an optimization perspective, adding decoder directions can strictly lower the $\ell_1$-regularized population risk, even when a basis can already reconstruct the feature exactly. Motivated by these results, we introduce Subspace-Aware Sparse Autoencoders (SASA), which replace single-vector decoders with learned subspaces, enforce sparsity through Top-$s$ group gating, and adapt group rank with nuclear-norm regularization. Under an idealized single-feature model, we prove that the SASA objective is minimized by a single group whose reconstruction map recovers the feature subspace. We also derive polynomial sample complexity bounds for subspace estimation within a group and a lower bound on the samples needed to observe every atom in a fixed fragmented dictionary. Experiments on GPT-2 and Mistral-7B show reduced absorption compared with SAEs. Matched-budget GPT-2 comparisons show lower absorption for concept families and more accurate prediction of their members using a small number of latent coordinates, at a reconstruction cost. The code is available at https://github.com/arshandalili/sasa.

==> tables/efficiency.tex <==
\begin{table}[tbp]
\centering
\caption{Training budget on GPT-2 layer~7 for dictionaries with $12{,}288$ decoder columns. Each cell gives the value at a checkpoint saved during training ($150\mathrm{M}$ tokens for the vector SAEs and $100\mathrm{M}$ for SASA) and at the end of training ($300\mathrm{M}$ tokens). Concept-family absorption is mean $\pm$ standard deviation over six evaluation seeds. Member prediction uses six decoder columns and averages three train--test splits.}
\label{tab:efficiency}
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{@{}lccc@{}}
\toprule
Model & CE score (\%) $\uparrow$ & Family absorption (\%) $\downarrow$ & Member prediction (\%) $\uparrow$ \\
\midrule
\multicolumn{4}{@{}l}{\emph{$\ell_0=30$}} \\
TopK & 98.6 / 98.7 & $46.6{\pm}7.7$ / $46.8{\pm}10.0$ & 53.3 / 51.6 \\
BatchTopK & 98.7 / 98.8 & $34.5{\pm}6.2$ / $37.3{\pm}5.7$ & 48.9 / 48.5 \\
Matryoshka & 98.6 / 98.7 & $32.9{\pm}9.0$ / $26.5{\pm}13.0$ & 54.4 / 52.7 \\
SASA & 95.5 / 95.8 & $4.0{\pm}1.0$ / $7.9{\pm}0.9$ & 71.2 / 69.2 \\
\midrule
\multicolumn{4}{@{}l}{\emph{$\ell_0=60$}} \\
TopK & 99.2 / 99.2 & $42.9{\pm}11.2$ / $43.4{\pm}10.1$ & 67.3 / 66.1 \\
BatchTopK & 99.2 / 99.3 & $44.0{\pm}5.7$ / $48.1{\pm}6.0$ & 54.8 / 56.0 \\
Matryoshka & 99.2 / 99.2 & $41.7{\pm}8.0$ / $45.9{\pm}8.3$ & 67.2 / 59.9 \\
SASA & 97.1 / 97.3 & $10.5{\pm}1.7$ / $5.5{\pm}2.2$ & 77.6 / 77.7 \\
\midrule
\multicolumn{4}{@{}l}{\emph{$\ell_0=120$}} \\
TopK & 99.5 / 99.5 & $51.0{\pm}11.0$ / $49.7{\pm}4.1$ & 65.4 / 66.1 \\
BatchTopK & 99.6 / 99.6 & $44.6{\pm}9.0$ / $52.2{\pm}3.6$ & 64.1 / 63.0 \\
Matryoshka & 99.5 / 99.5 & $48.5{\pm}15.2$ / $51.0{\pm}10.7$ & 53.3 / 57.7 \\
SASA & 98.3 / 98.5 & $19.9{\pm}3.3$ / $25.5{\pm}5.0$ & 79.1 / 78.2 \\
\midrule
\multicolumn{4}{@{}l}{\emph{$\ell_0=240$}} \\
TopK & 99.8 / 99.8 & $61.5{\pm}7.9$ / $59.1{\pm}9.4$ & 61.9 / 65.8 \\
BatchTopK & 99.8 / 99.8 & $59.2{\pm}9.2$ / $61.9{\pm}5.6$ & 41.6 / 46.1 \\
Matryoshka & 99.7 / 99.8 & $67.3{\pm}7.2$ / $73.2{\pm}7.3$ & 36.7 / 35.4 \\
SASA & 99.2 / 99.3 & $40.6{\pm}5.0$ / $36.6{\pm}8.3$ & 66.6 / 68.0 \\
\bottomrule
\end{tabular}
\end{table}

